Mixed-Profile Recovery of Hidden Permutation Iterates

For a uniformly random permutation $\pi$ on $[N]$, a learner observes $q$ i.i.d.\ labeled edges and then one nonadaptive batch of at most $b$ membership queries, and must output $m$ distinct-start pairs $(R_j,\pi^k(R_j))$. On the mixed profile $m=\lfloor N^\gamma\rfloor$, $h=\lfloor N^\delta\rfloor$, and $b=m-h$, with fixed $k\ge2$ and $0<\delta<\gamma<1$, we prove a sharp $0$--$1$ threshold at $Q(N)=\max\{(mN^{k-2})^{1/(k-1)},(hN^{k-1})^{1/k}\}$. For every fixed $\varepsilon>0$, an explicit learner succeeds with probability $1-o(1)$ above $(1+\varepsilon)Q(N)$, and every learner succeeds with probability $o(1)$ below $(1-\varepsilon)Q(N)$. The same sharp statement holds for independent budgets $b=O(m)$ when $b\ge m$ or $m-b=\Omega(m)$. The upper bound concentrates two passive prefix populations. The lower bound tracks batch collisions, queries whose images land back in the revealed domain, in a deterministic walk-capacity inequality, then applies a last-fresh-edge posterior bound. Thus the zero-collision union bound can fail before the sample threshold changes. A thin independent-budget regime remains open, where nonterminal collisions can contribute a comparable number of certificates. The results are information-theoretic and restricted to one nonadaptive batch; they do not address generalization, computation, total-variation graph sampling, or multi-round adaptivity.

==> template_core/color_tokens.tex <==
\RequirePackage{xcolor}
\definecolor{PaperInk}{HTML}{18232B}             
\definecolor{PaperMutedInk}{HTML}{5B6873}        
\definecolor{PaperRule}{HTML}{D1D8DE}            
\definecolor{PaperAccent}{HTML}{003155}          
\definecolor{PaperAccentDark}{HTML}{00223D}      
\definecolor{PaperAccentLight}{HTML}{E6EEF3}     
\definecolor{PaperAccentPale}{HTML}{F6F9FB}      
\definecolor{PaperNavigation}{HTML}{1B3F8D}      
\definecolor{PaperNavigationLight}{HTML}{E9EEFA} 
\definecolor{PaperDefinition}{HTML}{244117}      
\definecolor{PaperDefinitionLight}{HTML}{EEF2EA} 
\definecolor{PaperGold}{HTML}{C79C5E}            
\definecolor{PaperGoldLight}{HTML}{FAF3E8}       
\definecolor{PaperAlgorithmLight}{HTML}{F0F5F8} 
\definecolor{PaperLink}{HTML}{1B3F8D}            
\definecolor{PaperCitation}{HTML}{244117}        
\definecolor{PaperUrl}{HTML}{003155}             
\definecolor{PaperDraft}{HTML}{9A4F3D}           


==> template_core/layout.tex <==
\RequirePackage[margin=0.9in]{geometry}
\linespread{1.05}
\frenchspacing
\widowpenalty=10000
\clubpenalty=10000
\setlength{\emergencystretch}{3em}
\setlength{\parindent}{1.2em}
\setlength{\parskip}{0pt}


==> template_core/theorem_environments.tex <==
\usepackage{amsthm}
\usepackage{thm-restate}
\makeatletter
% amsthm already binds sibling theorem counters and display names. Avoid a
% second counter-alias registration in newer thmtools/amsthm combinations.
\renewcommand{\@counteralias}[2]{{%
  \def\@@gletover##1##2{%
    \expandafter\global\expandafter\let\csname ##1\expandafter\endcsname\csname ##2\endcsname}%
  \@ifundefined{c@#2}{\@nocounterr{#2}}{%
    \@@gletover{c@#1}{c@#2}%
    \@@gletover{the#1}{the#2}%
    \@@gletover{theH#1}{theH#2}%
    \@ifpackageloaded{cleveref}{%
      \edef\aliasctr@temp{%
        \noexpand\cref@resetby{#2}{\noexpand\cref@result}}%
      \aliasctr@temp
      \ifx\cref@result\relax\else
        \cref@addtoreset{#1}{\cref@result}%
      \fi
    }{}%
    \@@gletover{p@#1}{p@#2}%
    \expandafter\global\expandafter\def\csname cl@#1\expandafter\endcsname
      \expandafter{\csname cl@#2\endcsname}%
  }%
}}
\makeatother
\usepackage[most]{tcolorbox}
\usepackage{needspace}

\newcommand{\PaperTheoremHeadFont}{\PaperHeadingFont\bfseries}
\newcommand{\PaperTheoremBodyFont}{\itshape}
\newcommand{\PaperDefinitionHeadFont}{\PaperHeadingFont\bfseries}
\newcommand{\PaperDefinitionBodyFont}{\normalfont}
\newcommand{\PaperRemarkHeadFont}{\PaperHeadingFont\itshape}
\newcommand{\PaperRemarkBodyFont}{\normalfont}
\newtheoremstyle{paperplain}
  {0pt}{0pt}{\PaperTheoremBodyFont}{0pt}{\PaperTheoremHeadFont}{.}{0.5em}{}
\newtheoremstyle{paperdefinition}
  {0pt}{0pt}{\PaperDefinitionBodyFont}{0pt}{\PaperDefinitionHeadFont}{.}{0.5em}{}
\newtheoremstyle{paperremark}
  {0pt}{0pt}{\PaperRemarkBodyFont}{0pt}{\PaperRemarkHeadFont}{.}{0.5em}{}

\makeatletter
\makeatother

\theoremstyle{paperplain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{fact}[theorem]{Fact}

\theoremstyle{paperdefinition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{openproblem}[theorem]{Open Problem}

\theoremstyle{paperremark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}

\newcommand{\PaperPlainBlockStyle}[1]{%
  \tcolorboxenvironment{#1}{
    enhanced jigsaw,
    boxrule=0pt,
    colframe=PaperAccent,
    colback=PaperAccentPale,
    arc=1.2mm,
    left=7pt,
    right=7pt,
    top=4pt,
    bottom=4pt,
    before=\Needspace{12\baselineskip},
    before skip=8pt,
    after skip=8pt
  }
}
\newcommand{\PaperDefinitionBlockStyle}[1]{%
  \tcolorboxenvironment{#1}{
    enhanced jigsaw,
    boxrule=0pt,
    colframe=PaperDefinition,
    colback=PaperDefinitionLight,
    arc=1.2mm,
    left=7pt,
    right=7pt,
    top=4pt,
    bottom=4pt,
    before=\Needspace{12\baselineskip},
    before skip=8pt,
    after skip=8pt
  }
}
\newcommand{\PaperRemarkBlockStyle}[1]{%
  \tcolorboxenvironment{#1}{
    enhanced jigsaw,
    boxrule=0pt,
    colframe=PaperRule,
    colback=white,
    arc=1.2mm,
    left=7pt,
    right=7pt,
    top=4pt,
    bottom=4pt,
    before=\Needspace{10\baselineskip},
    before skip=7pt,
    after skip=7pt
  }
}

\floatstyle{ruled}
\restylefloat{algorithm}
\newcommand{\PaperAlgorithmLabelFont}{\bfseries}
\newcommand{\PaperAlgorithmCaptionFont}{\small\PaperBodyFont\color{PaperInk}}
\newcommand{\PaperAlgorithmBodyFont}{\small\PaperBodyFont\color{PaperInk}}
\newcommand{\PaperAlgorithmLineNumberFont}{\footnotesize\PaperBodyFont\color{PaperMutedInk}}
\newcommand{\PaperAlgorithmCommentFont}{\footnotesize\PaperBodyFont\itshape\color{PaperMutedInk}}
\newcommand{\PaperAlgorithmInputFont}{\PaperBodyFont\bfseries\color{PaperNavigation}}
\newcommand{\PaperAlgorithmOutputFont}{\PaperBodyFont\bfseries\color{PaperNavigation}}
\newcommand{\PaperAlgorithmKeywordFont}{\PaperBodyFont\bfseries\color{PaperInk}}
\newcommand{\PaperAlgorithmProcedureFont}{\PaperBodyFont\mdseries\color{PaperInk}}
\newcommand{\PaperAlgorithmInputText}{Input:}
\newcommand{\PaperAlgorithmOutputText}{Output:}
\DeclareCaptionFont{paperalgorithmlabel}{\PaperAlgorithmLabelFont}
\DeclareCaptionFont{paperalgorithmcaption}{\PaperAlgorithmCaptionFont}
\captionsetup[algorithm]{font=paperalgorithmcaption,labelfont=paperalgorithmlabel,labelsep=colon,skip=5pt,singlelinecheck=false,justification=raggedright}
\algrenewcommand{\algorithmicrequire}{\PaperAlgorithmInputFont\PaperAlgorithmInputText}
\algrenewcommand{\algorithmicensure}{\PaperAlgorithmOutputFont\PaperAlgorithmOutputText}
\algrenewcommand{\algorithmiccomment}[1]{\hfill{\PaperAlgorithmCommentFont\(\triangleright\)~#1}}
\algrenewcommand{\alglinenumber}[1]{{\PaperAlgorithmLineNumberFont #1}}
\algrenewcommand{\algorithmicif}{\PaperAlgorithmKeywordFont if}
\algrenewcommand{\algorithmicthen}{\PaperAlgorithmKeywordFont then}
\algrenewcommand{\algorithmicelse}{\PaperAlgorithmKeywordFont else}
\algrenewcommand{\algorithmicfor}{\PaperAlgorithmKeywordFont for}
\algrenewcommand{\algorithmicwhile}{\PaperAlgorithmKeywordFont while}
\algrenewcommand{\algorithmicdo}{\PaperAlgorithmKeywordFont do}
\algrenewcommand{\algorithmicend}{\PaperAlgorithmKeywordFont end}
\algrenewcommand{\algorithmicprocedure}{\PaperAlgorithmKeywordFont procedure}
\algrenewcommand{\textproc}[1]{{\PaperAlgorithmProcedureFont #1}}
\algrenewcommand{\algorithmicreturn}{\PaperAlgorithmKeywordFont return}
\AtBeginEnvironment{algorithmic}{\PaperAlgorithmBodyFont}
\newenvironment{paperalgorithmic}[1][1]{\begin{algorithmic}[#1]}{\end{algorithmic}}

\AtBeginDocument{
  \PaperPlainBlockStyle{theorem}
  \PaperPlainBlockStyle{lemma}
  \PaperPlainBlockStyle{proposition}
  \PaperPlainBlockStyle{corollary}
  \PaperPlainBlockStyle{conjecture}
  \PaperPlainBlockStyle{fact}
  \PaperDefinitionBlockStyle{definition}
  \PaperDefinitionBlockStyle{assumption}
  \PaperDefinitionBlockStyle{example}
  \PaperDefinitionBlockStyle{problem}
  \PaperDefinitionBlockStyle{openproblem}
  \PaperRemarkBlockStyle{remark}
  \PaperRemarkBlockStyle{claim}
}


==> template_core/typography.tex <==
\RequirePackage{iftex}
\ifPDFTeX
  \RequirePackage[T1]{fontenc}
  \RequirePackage[utf8]{inputenc}
  \RequirePackage{lmodern}
\else
  \RequirePackage{fontspec}
  \setmainfont[Path=/usr/local/texlive/2025/texmf-dist/fonts/opentype/public/lm/,Extension=.otf,BoldFont=lmroman10-bold,ItalicFont=lmroman10-italic,BoldItalicFont=lmroman10-bolditalic,SmallCapsFont=lmromancaps10-regular]{lmroman10-regular}
  \setsansfont[Path=/usr/local/texlive/2025/texmf-dist/fonts/opentype/public/lm/,Extension=.otf,BoldFont=lmsans10-bold,ItalicFont=lmsans10-oblique,BoldItalicFont=lmsans10-boldoblique]{lmsans10-regular}
  \setmonofont[Path=/usr/local/texlive/2025/texmf-dist/fonts/opentype/public/lm/,Extension=.otf]{lmmono10-regular}
\fi
\newcommand{\PaperBodyFont}{\rmfamily}
\newcommand{\PaperHeadingFont}{\sffamily}
\newcommand{\PaperCaptionFont}{\sffamily}
\newcommand{\PaperCodeFont}{\ttfamily}

